IntentsKB: A Knowledge Base of Entity-Oriented Search Intents

We address the problem of constructing a knowledge base of entity-oriented search intents. Search intents are defined on the level of entity types, each comprising of a high-level intent category (property, website, service, or other), along with a cluster of query terms used to express that intent. These machine-readable statements can be leveraged in various applications, e.g., for generating entity cards or query recommendations. By structuring service-oriented search intents, we take one step towards making entities actionable. The main contribution of this paper is a pipeline of components we develop to construct a knowledge base of entity intents. We evaluate performance both component-wise and end-to-end, and demonstrate that our approach is able to generate high-quality data.

==> cikm2018-intents-kb-04_table.tex <==
% Table of features for refiner categorization

% Abbreviated table commented below

% Original full table (1 row per feature) commented below

%
\begin{table*}[!ht]
  \centering
  \caption{Features for refiners categorization.}
  \vspace{-0.03in}
  \label{table:features}
%  \captionshrink
  \footnotesize
  \begin{tabular}{ l p{14cm} l }
    \toprule
	\#  & Description & Value \\ % & \dg{Source} 
    \midrule
    \multicolumn{3}{l}{\emph{Group I - Lexical features}} \\
    1 & Length of the top result title, in characters & $\{1, \dots, \infty\}$ \\
    2 & Avg. length of the 10 result titles, in characters & $\{1, \dots, \infty\}$ \\
    3 & Length of the top result snippet, in characters & $\{1, \dots, \infty\}$ \\
    4 & Avg. length of the 10 result snippets, in characters & $\{1, \dots, \infty\}$ \\
    5 & Number of `/' in the top result URL & $\{0, \dots, \infty\}$ \\
    6 & avg. number of `/' in the top 10 result URLs & $\{0, \dots, \infty\}$ \\
    7 & size of the URL domains set among all top 10 result URLs. & $\{1, \dots, 10\}$ \\
    8 & Jaro distance between the refiner and the top result URL & $[0..1]$ \\
    9 & Avg. Jaro distance between the refiner and each of the top 10 result URLs & $[0..1]$ \\
    10 & Avg. Jaro distance between all the top 10 result URLs & $[0..1]$ \\
    11-13 & $\{$Max., Min., Mean$\}$ aggregated term-to-term Jaro distance between the refiner and the top result title & $[0..1]$ \\
    14-16 & Avg. $\{$max., min., mean$\}$ aggregated term-to-term Jaro distance between the refiner and the top 10 result titles & $[0..1]$ \\
    \midrule
%    \multicolumn{3}{l}{\emph{Group II - Mark-up features}} \\
%    17-22 & No. of results, among the top 10, where $t$ OG type occurs in the result pagemap metatags, $t \in \{$\texttt{music}, \texttt{video}, \texttt{article}, \texttt{book}, \texttt{profile}, \texttt{website}$\}$  & $\{0, \dots, 10\}$ \\
%    23-31 & No. of results, among the top 10, where $t$ Tumblr API type occurs in the result pagemap metatags, $t \in \{$\texttt{profile}, \texttt{text}, \texttt{photo}, \texttt{quote}, \texttt{link}, \texttt{chat}, \texttt{audio}, \texttt{video}, \texttt{answer}$\}$ & $\{0, \dots, 10\}$ \\
%    32-38 & No. of results, among the top 10, where $t$ prefix occurs in the result pagemap metatags, $t \in \{$\texttt{apple-itunes-app}, \texttt{apple-mobile-web-app}, \texttt{tumblr:app\_id}, \texttt{al:android}, \texttt{al:ios}, \texttt{al:web}, \texttt{fb:app\_id}$\}$  & $\{0, \dots, 10\}$ \\
%    39-40 & No. of results, among the top 10, where $t$ occurs in the result pagemap, $t \in \{$\texttt{mobileapplication}, \texttt{videoobject}$\}$  & $\{0, \dots, 10\}$ \\
%    \midrule
    \multicolumn{3}{l}{\emph{Group II - Semantic features}} \\
    41 & Cosine sim. between the refiner and type \emph{word2vec} vectors aggregated over all their resp. terms & $[0..1]$ \\
    \bottomrule
  \end{tabular}
\end{table*}
%


% -----------------
% Abbreviated table commented below
%
%\begin{table*}[!ht]
%  \centering
%  \caption{Features for refiners categorization.}
%  \vspace{-0.03in}
%  \label{table:features}
%  \captionshrink
%  \footnotesize
%  \begin{tabular}{ l p{14cm} l }
%    \toprule
%	\#  & Description & Value \\ % & \dg{Source} 
%    \midrule
%    \multicolumn{3}{l}{\emph{I - Lexical features}} \\
%    1 & Length of the top result title, in characters & $\{1, \dots, \infty\}$ \\
%    2 & Avg. length of the 10 result titles, in characters & $\{1, \dots, \infty\}$ \\
%    3 & Length of the top result snippet, in characters & $\{1, \dots, \infty\}$ \\
%    4 & Avg. length of the 10 result snippets, in characters & $\{1, \dots, \infty\}$ \\
%    5 & Number of `/' in the top result URL & $\{0, \dots, \infty\}$ \\
%    6 & avg. number of `/' in the top 10 result URLs & $\{0, \dots, \infty\}$ \\
%    7 & size of the URL domains set among all top 10 result URLs. & $\{1, \dots, 10\}$ \\
%    8 & Jaro distance between the refiner and the top result URL & $[0..1]$ \\
%    9 & Avg. Jaro distance between the refiner and each of the top 10 result URLs & $[0..1]$ \\
%    10 & Avg. Jaro distance between all the top 10 result URLs & $[0..1]$ \\
%    11-13 & $\{$Max., Min., Mean$\}$ aggregated term-to-term Jaro distance between the refiner and the top result title & $[0..1]$ \\
%    14-16 & Avg. $\{$max., min., mean$\}$ aggregated term-to-term Jaro distance between the refiner and the top 10 result titles & $[0..1]$ \\
%    \midrule
%    \multicolumn{3}{l}{\emph{II - Mark-up features}} \\
%    17-22 & No. of results, among the top 10, where $t$ OG type occurs in the result pagemap metatags, $t \in \{$\texttt{music}, \texttt{video}, \texttt{article}, \texttt{book}, \texttt{profile}, \texttt{website}$\}$  & $\{0, \dots, 10\}$ \\
%    23-31 & No. of results, among the top 10, where $t$ Tumblr API type occurs in the result pagemap metatags, $t \in \{$\texttt{profile}, \texttt{text}, \texttt{photo}, \texttt{quote}, \texttt{link}, \texttt{chat}, \texttt{audio}, \texttt{video}, \texttt{answer}$\}$ & $\{0, \dots, 10\}$ \\
%    32-38 & No. of results, among the top 10, where $t$ prefix occurs in the result pagemap metatags, $t \in \{$\texttt{apple-itunes-app}, \texttt{apple-mobile-web-app}, \texttt{tumblr:app\_id}, \texttt{al:android}, \texttt{al:ios}, \texttt{al:web}, \texttt{fb:app\_id}$\}$  & $\{0, \dots, 10\}$ \\
%    39-40 & No. of results, among the top 10, where $t$ occurs in the result pagemap, $t \in \{$\texttt{mobileapplication}, \texttt{videoobject}$\}$  & $\{0, \dots, 10\}$ \\
%    \midrule
%    \multicolumn{3}{l}{\emph{III - Semantic features}} \\
%    41 & Cosine sim. between the refiner and type \emph{word2vec} vectors aggregated over all their resp. terms & $[0..1]$ \\
%    \bottomrule
%  \end{tabular}
%\end{table*}
%


% -----------------
% Original full table (1 row per feature)

%
%\begin{table*}[!ht]
%  \centering
%  \caption{Features for refiners categorization.}
%  \vspace{-0.03in}
%  \label{table:features}
%  \captionshrink
%  \footnotesize
%  \begin{tabular}{ l p{14cm} l }
%    \toprule
%	\#  & Description & Value \\ % & \dg{Source} 
%    \midrule
%    \multicolumn{3}{l}{\emph{I - Lexical features}} \\
%    1 & Length of the top result title, in characters & $\{1, \dots, \infty\}$ \\
%    2 & Avg. length of the 10 result titles, in characters & $\{1, \dots, \infty\}$ \\
%    3 & Length of the top result snippet, in characters & $\{1, \dots, \infty\}$ \\
%    4 & Avg. length of the 10 result snippets, in characters & $\{1, \dots, \infty\}$ \\
%    5 & Number of `/' in the top result URL & $\{0, \dots, \infty\}$ \\
%    6 & avg. number of `/' in the top 10 result URLs & $\{0, \dots, \infty\}$ \\
%    7 & size of the URL domains set among all top 10 result URLs. & $\{1, \dots, 10\}$ \\
%    8 & Jaro distance between the refiner and the top result URL & $[0..1]$ \\
%    9 & Avg. Jaro distance between the refiner and each of the top 10 result URLs & $[0..1]$ \\
%    10 & Avg. Jaro distance between all the top 10 result URLs & $[0..1]$ \\
%    11 & Max. aggregated term-to-term Jaro distance between the refiner and the top result title & $[0..1]$ \\
%    12 & Min. aggregated term-to-term Jaro distance between the refiner and the top result title & $[0..1]$ \\
%    13 & Mean aggregated term-to-term Jaro distance between the refiner and the top result title & $[0..1]$ \\
%    14 & Avg. max. aggregated term-to-term Jaro distance between the refiner and the top 10 result titles & $[0..1]$ \\
%    15 & Avg. min. aggregated term-to-term Jaro distance between the refiner and the top 10 result titles & $[0..1]$ \\
%    16 & Avg. mean aggregated term-to-term Jaro distance between the refiner and the top 10 result titles & $[0..1]$ \\
%    \midrule
%    \multicolumn{3}{l}{\emph{II - Mark-up features}} \\
%    17 & No. of results, among the top 10, where \texttt{music} OG type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    18 & No. of results, among the top 10, where \texttt{video} OG type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    19 & No. of results, among the top 10, where \texttt{article} OG type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    20 & No. of results, among the top 10, where \texttt{book} OG type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    21 & No. of results, among the top 10, where \texttt{profile} OG type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    22 & No. of results, among the top 10, where \texttt{website} OG type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    23 & No. of results, among the top 10, where \texttt{profile} Tumblr API type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    24 & No. of results, among the top 10, where \texttt{text} Tumblr API type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    25 & No. of results, among the top 10, where \texttt{photo} Tumblr API type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    26 & No. of results, among the top 10, where \texttt{quote} Tumblr API type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    27 & No. of results, among the top 10, where \texttt{link} Tumblr API type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    28 & No. of results, among the top 10, where \texttt{chat} Tumblr API type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    29 & No. of results, among the top 10, where \texttt{audio} Tumblr API type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    30 & No. of results, among the top 10, where \texttt{video} Tumblr API type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    31 & No. of results, among the top 10, where \texttt{answer} Tumblr API type occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    32 & No. of results, among the top 10, where \texttt{apple-itunes-app} prefix occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    33 & No. of results, among the top 10, where \texttt{apple-mobile-web-app} prefix occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    34 & No. of results, among the top 10, where \texttt{tumblr:app\_id} prefix occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    35 & No. of results, among the top 10, where \texttt{al:android} prefix occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    36 & No. of results, among the top 10, where \texttt{al:ios} prefix occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    37 & No. of results, among the top 10, where \texttt{al:web} prefix occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    38 & No. of results, among the top 10, where \texttt{fb:app\_id} prefix occurs in the result pagemap metatags  & $\{0, \dots, 10\}$ \\
%    39 & No. of results, among the top 10, where \texttt{mobileapplication} occurs in the result pagemap  & $\{0, \dots, 10\}$ \\
%    40 & No. of results, among the top 10, where \texttt{videoobject} occurs in the result pagemap  & $\{0, \dots, 10\}$ \\    \midrule
%    \multicolumn{3}{l}{\emph{III - Semantic features}} \\
%    41 & Cosine sim. between the refiner and type \emph{word2vec} vectors aggregated over all their resp. terms & $[0..1]$ \\
%    \bottomrule
%  \end{tabular}
%\end{table*}
%

